Galaxy And Mass Assembly (GAMA): Stellar mass growth of spiral galaxies in the cosmic web

We look for correlated changes in stellar mass and star formation rate along filaments in the cosmic web by examining the stellar masses and UV-derived star formation rates (SFR) of 1,799 ungrouped and unpaired spiral galaxies that reside in filaments. We devise multiple distance metrics to characterise the complex geometry of filaments, and find that galaxies closer to the cylindrical centre of a filament have higher stellar masses than their counterparts near the periphery of filaments, on the edges of voids. In addition, these peripheral spiral galaxies have higher specific star formation rates (SSFR) at a given mass. Complementing our sample of filament spiral galaxies with spiral galaxies in tendrils and voids, we find that the average SFR of these objects in different large scale environments are similar to each other with the primary discriminant in SFR being stellar mass, in line with previous works. However, the distributions of SFRs are found to vary with large-scale environment. Our results thus suggest a model in which in addition to stellar mass as the primary discriminant, the large-scale environment is imprinted in the SFR as a second order effect. Furthermore, our detailed results for filament galaxies suggest a model in which gas accretion from voids onto filaments is primarily in an orthogonal direction. Overall, we find our results to be in line with theoretical expectations of the thermodynamic properties of the intergalactic medium in different large-scale environments.

==> views.tex <==
VIEW={Filament overview}
  COO=-18.245609283447266 2.6941616535186768 225.68634033203125
  C2C=0.05373663082718849 -0.612947940826416 -0.7882938385009766
  ROO=26.181367215212664
  ROLL=-85.13778890983203
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END
VIEW={Spiral galaxy}
  COO=-15.76726245880127 0.9822713136672974 226.95201110839844
  C2C=0.1651933342218399 -0.69652259349823 -0.6982603669166565
  ROO=7.904951750422875
  ROLL=-89.78761777223662
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END
VIEW={Filament centre}
  COO=-17.52692413330078 7.786470890045166 225.4387664794922
  C2C=-0.8985725045204163 0.18113812804222107 -0.39969557523727417
  ROO=5.871931207945121
  ROLL=36.246543510072044
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END
VIEW={Closest group}
  COO=-13.436412811279297 -0.4514266550540924 228.46006774902344
  C2C=0.12239710986614227 -0.8798693418502808 -0.45918288826942444
  ROO=7.100187497954087
  ROLL=-84.32678590816305
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END
VIEW={Closest backbone group}
  COO=-17.246627807617188 4.145991325378418 226.4353790283203
  C2C=0.16102659702301025 0.672727644443512 0.7221550941467285
  ROO=7.10019421378987
  ROLL=80.71137553517853
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END
VIEW={Most massive group}
  COO=-21.831069946289062 1.6222901344299316 235.14584350585938
  C2C=-0.5899394154548645 0.2599763572216034 0.7644500732421875
  ROO=8.118525816044514
  ROLL=-116.95964025292143
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END

